Optimization Modulo the Theories of Signed Bit-Vectors and Floating-Point Numbers

Optimization Modulo Theories (OMT) is an important extension of SMT which allows for finding models that optimize given objective functions, typically consisting in linear-arithmetic or pseudo-Boolean terms. However, many SMT and OMT applications, in particular from SW and HW verification, require handling bit-precise representations of numbers, which in SMT are handled by means of the theory of Bit-Vectors (BV) for the integers and that of Floating-Point Numbers (FP) for the reals respectively. Whereas an approach for OMT with (unsigned) BV has been proposed by Nadel & Ryvchin, unfortunately we are not aware of any existing approach for OMT with FP. In this paper we fill this gap. We present a novel OMT approach, based on the novel concept of attractor and dynamic attractor, which extends the work of Nadel & Ryvchin to signed BV and, most importantly, to FP. We have implemented some OMT(BV) and OMT(FP) procedures on top of OptiMathSAT and tested the latter ones on modified problems from the SMT-LIB repository. The empirical results support the validity and feasibility of the novel approach.

==> Makefile <==
LATEX=pdflatex
SOURCE=main
JOB_NAME=main_long

.PHONY:

default: short

all: long-bib short-bib

clean:
	$(RM) main.pdf main_long.pdf  *.ps *.dvi *.aux *.toc *.log *.bak *.backup *.blg *.bbl *.cut *~

short: set_short
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

short-bib: set_short
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	bibtex   $(JOB_NAME)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

long: set_long
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

long-bib: set_long
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	bibtex   $(JOB_NAME)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

upload:
	git push

set_appendix: force
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{true}/\\\\newcommand{\\\\withproofs}{false}/g" options.tex'

set_proofs: force
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{false}/\\\\newcommand{\\\\withproofs}{true}/g" options.tex'

set_short: force
	$(eval JOB_NAME=main)
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{true}/\\\\newcommand{\\\\withproofs}{false}/g" options.tex'
	bash -c 'sed -i "s/\\\\newcommand{\\\\longversion}{true}/\\\\newcommand{\\\\longversion}{false}/g" options.tex'

set_long: force
	$(eval JOB_NAME=main_long)
	bash -c 'sed -i "s/\\\\newcommand{\\\\longversion}{false}/\\\\newcommand{\\\\longversion}{true}/g" options.tex'
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{false}/\\\\newcommand{\\\\withproofs}{true}/g" options.tex'

force:
	#git update-index --assume-unchanged options.tex


==> src/proofs/tf_bv_long.tex <==
We demonstrate that Theorem~\ref{thm:bvoptnasc} holds, for both signed
and unsigned \bv objectives, using the following argument.

\medskip

\begin{proof}
Let $\pair{\varphi}{\cost}$ be an \omtbv problem where $\cost$ is
a \bv objective to be minimized and $\attr$ is its attractor, that
is, the smallest value that can be represented with a \bv value of
the same type of \cost.
%
Let $\attreq{}$ be the corresponding vector of attractor equalities s.t.,
for each $i$, $\attreq{i} = (\costbit{i} = \attrbit{i})$.
%
Finally, let $\calm$ be a a model of $\varphi$ which {\em lexicographically
maximizes} $\attreq{}$, where $\mu$ is the corresponding (complete) truth assignment
over the Boolean abstraction of $\varphi$, $\tau_n \defas \restr{\mu}{n}$ is
the restriction of $\mu$ over the bits of $\cost$ and $\calm(\cost)$ is the model
value of $\cost$, computed with Equation~\eqref{eq:bv-unsigned} if $\cost$ is an
\emph{unsigned} \bv objective and with Equation~\eqref{eq:bv-signed} otherwise.
%
By definition, model $\calm$ is an optimal solution for $\pair{\varphi}{\cost}$
if there exists no other model $\calm'$ s.t. $\calm'$ satisfies $\varphi$
and $\calm'(\cost) < \calm(\cost)$. Hence, we prove that Theorem~\ref{thm:bvoptnasc}
holds showing that no such $\calm'$ can exist.

Assume (for the sake of contradiction), that there exists a model $\calm'$,
corresponding to a (complete) truth assignment $\mu'$, s.t. $\calm'$
satisfies $\varphi$ and $\calm'(\cost) < \calm(\cost)$.
%
Let $\tau_n' \defas \restr{\mu'}{n}$ be the restriction of $\mu'$ over
the bits of $\cost$.
%
Since $\calm'(\cost) \neq \calm(\cost)$, by Equations~\eqref{eq:bv-unsigned}-\eqref{eq:bv-signed}
there must be at least one index $i$ for which $\mu(\costbit{i}) \neq \mu'(\costbit{i})$.
%
Let $m$ be the smallest index $i$, from $0$ to $n-1$, s.t.
$\mu(\costbit{i}) \neq \,u'(\costbit{i})$.
%
We set $\tau_m \defas \restr{\mu}{m}$, $\tau_{m+1} \defas \restr{\mu}{m+1}$ and
$\tau_{m+1}' \defas \restr{\mu'}{m+1}$. Then, $\tau_m \subset \tau_{m+1}$,
$\tau_m \subset \tau_{m+1}'$, $\tau_{m+1} \neq \tau_{m+1}'$. In particular,
$\tau_{m+1}(\costbit{m}) = \neg \tau_{m+1}'(\costbit{m})$ and therefore
$\tau_{m+1} \models \attreq{m}$ if $\tau_{m+1}' \models \neg \attreq{m}$, and vice versa.

We split our proof in two parts: in the first we consider of an \emph{unsigned} \bv goal,
while in the second part we consider the case of a \emph{signed} \bv objective.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

\noindent
\textbf{\textsc{case I}: $\cost$ is an unsigned \bv goal.}
%
Then, we distinguish two sub-cases.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

In the first case, $\tau_{m+1} \models \neg \attreq{m}$ and $\tau_{m+1}' \models \attreq{m}$.
%
From $\tau_{m+1} \models \neg \attreq{m}$ and the fact that, by
Theorem~\ref{thm:bvoptnasc}, $\mu$ {\em lexicographically maximizes}
$\attreq{}$, we derive that $\varphi \wedge \tau_m \models \neg \attreq{m}$.
%
Because $\tau_m \subset \tau_{m+1}' \subseteq \mu'$ and $\tau_{m+1}' \models \attreq{m}$,
we conclude that $\varphi \wedge \mu' \models \false$ and that $\calm'$ cannot be
a satisfiable model of $\varphi$, contradicting the initial assumption.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

In the second case, $\tau_{m+1} \models \attreq{m}$ and $\tau_{m+1}' \models \neg \attreq{m}$.
%
For $\calm'(\cost) < \calm(\cost)$ to hold, the difference
$\Delta \defas \calm'(\cost) - \calm(\cost)$ computed in
Equation~\eqref{eq:bv-proof-2} must be smaller than zero.
%
\begin{equation}
\scriptsize
\label{eq:bv-proof-2}
\begin{aligned}
%& \calm'[\cost] - \calm[\cost] & = & \:\:
& \Delta & = & \:\:
    \sum_{i=0}^{i=n-1} (2^{n-1-i} \cdot \textsc{ite}(\mu'(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}})) - {}\\
& & {} & \:\: \sum_{i=0}^{i=n-1} (2^{n-1-i} \cdot \textsc{ite}(\mu(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}})) \\
& &= & \:\:
    2^{n-1-m} \cdot (\overline{\attrbit{m}} + \attrbit{m}) + {}\\
& & {} & \:\: \sum_{i=m+1}^{i=n-1} (2^{n-1-i} \cdot \textsc{ite}(\mu'(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}})) - {} \\
& & & \:\:
    \sum_{i=m+1}^{i=n-1} (2^{n-1-i} \cdot \textsc{ite}(\mu(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}})) \\
& &= & \:\:
    2^{n-1-m} + {} \\
& & {} & \:\:
 \sum_{i=m+1}^{i=n-1} (2^{n-1-i} \cdot (\textsc{ite}(\mu'(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}}) - {}
    \textsc{ite}(\mu(\attreq{i}), \attrbit{i}, \overline{\attrbit{i}})) \\
\end{aligned}
\end{equation}

\noindent
It can be seen that there cannot exist any pair of assignments $\pair{\mu}{\mu'}$ s.t.
$\calm'[\cost] < \calm[\cost]$, because for any positive $k \defas n - 1 - m$, the
value $2^k$ (a.k.a. $2^{n-1-m}$) is strictly larger than $\sum_{i=0}^{i=k-1} 2^i$
(a.k.a. $\sum_{i=m+1}^{i=n-1} 2^{n-1-i}$).
%
This contradicts the initial assumption that $\calm'(\cost)< \calm(\cost)$.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

\noindent
\textbf{\textsc{case II}: \cost is a signed \bv goal.}
%
Then, we distinguish --once again-- two sub-cases.

In the first case, $m$ is larger than $0$. Therefore, $\calm(\cost)$
and $\calm'(\cost)$ are either both negative- or both positive-valued.
%
Looking at Equation~\eqref{eq:bv-signed}, which adheres to the \emph{two's
complement} representation rules, we observe that the \emph{sign bit} results
in a constant-valued displacement of the model value $\calm(\cost)$, which is
otherwise equal to the one computed by Equation~\eqref{eq:bv-unsigned}.
%
Since the value assigned to $\costbit{0}$ by $\calm$ and $\calm'$ provides
the same (fixed) contribution to the value of $\cost$, we can ignore the
\emph{sign bit} and restrict our focus on the remaining $n-1$ bits.
%
In this way, we obtain a new $\cost' \defas [\costbit{1}, ..., \costbit{n-1}]$,
a new $\attr' \defas [\attrbit{1}, ..., \attrbit{n-1}]$ and
a new $\attreq{}' \defas [(\costbit{1} = \attrbit{1}), ..., (\costbit{n-1} = \attrbit{n-1})]$.
%
For all intents and purposes, following the \emph{two's complement} representation,
the new goal $\cost'$ can be considered as an \emph{unsigned} \bv goal as it was
obtained by dropping the \emph{sign bit} from $\cost$.
%
As a consequence, we can apply the same argument illustrated in \textbf{\textsc{case I}}
over the new $\cost'$, $\attr'$ and $\attreq{}'$ to prove Theorem~\ref{thm:bvoptnasc}.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

In the second case, $m$ is equal to $0$.
%
By assumption, $\calm'(\cost) < \calm(\cost)$ so we have that $\calm'(\cost) < 0$
and $\calm(\cost) \geq 0$.
%
Given that $\cost$ is being minimized, the value of $\attrbit{0}$ is equal to $1$.
Substituting this value and Equation~\eqref{eq:bv-signed} inside both disequalities
$\calm(\cost) \geq 0$ and $\calm'(\cost) < 0$, we immediately get that
$\mu \models \neg \attreq{0}$ and that $\mu' \models \attreq{0}$.
%
Since, by Theorem~\ref{thm:bvoptnasc}, $\mu$ {\em lexicographically maximizes}
$\attreq{}$ and $\restr{\mu}{0} = \emptyset$, then it must be the case that
$\varphi \models \neg \attreq{0}$.
%
Therefore, we conclude that $\varphi \wedge \mu' \models \false$ and that $\calm'$
cannot be a satisfiable model of $\varphi$, contradicting the initial assumption.

(Dual for maximization.)
\end{proof}


==> src/proofs/tf_fp_old.tex <==
\begin{proof}
Let $\pair{\vinonan}{\cost}$, $\calm$, $\tau_0, \tau_1, ..., \tau_n$ and
$\dcala{}$ be as in Theorem~\ref{thm:fpopt1}.
%
Since both $\tau_n$ and $\calm$ lexicographically maximize $\dcala{}$, we
immediately notice that --for each $k\in[0..n]$-- $\tau_k = \restr{\mu}{k}$,
where $\mu$ is the (complete) truth assignment --over the Boolean abstraction
of $\vinonan$-- corresponding to $\calm$.

By definition, $\calm$ is an optimal solution for $\pair{\vinonan}{\cost}$ iff
there exists no other model $\calm'$ s.t. $\calm'$ satisfies $\vinonan$ and
$\calm'(\cost) < \calm(\cost)$. Hence, we prove that Theorem~\ref{thm:fpopt1}
holds showing that no such $\calm'$ can exist.

Assume (for the sake of contradiction), that there exists a model $\calm'$,
corresponding to a (complete) truth assignment $\mu'$ s.t. $\calm'$ satisfies
$\vinonan$ and $\calm'(\cost) < \calm(\cost)$.
%
Since $\calm'(\cost) \neq \calm(\cost)$, there must be at least one index $i$ for
which $\mu(\costbit{i}) \neq \mu'(\costbit{i})$. Let \minidx be the smallest index
$i$, from $0$ to $n-1$, s.t. $\mu(\costbit{i}) \neq \mu'(\costbit{i})$.
%
We set $\tau_{\minidx} \defas \restr{\mu}{\minidx}$,
$\tau_{\minidx+1} \defas \restr{\mu}{\minidx+1}$ and
$\tau_{\minidx+1}' \defas \restr{\mu'}{\minidx+1}$.
%
Then, $\tau_{\minidx} \subset \tau_{\minidx+1}$, $\tau_{\minidx} \subset \tau_{\minidx+1}'$,
$\tau_{\minidx+1} \neq \tau_{\minidx+1}'$. In particular,
$\tau_{\minidx+1}[\minidx] = \overline{\tau_{\minidx+1}'[\minidx]}$
and therefore $\tau_{\minidx+1} \models \dattreq{\tau_{\minidx}}{\minidx}$ if
$\tau_{\minidx+1}' \models \neg \dattreq{\tau_{\minidx}}{\minidx}$, and vice versa.

Then, we distinguish two cases.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

In the first case, $\tau_{\minidx+1}[\minidx] = \overline{\dattr{\tau_{\minidx}}{\minidx}}$
and $\tau_{\minidx+1}'[\minidx] = \dattr{\tau_{\minidx}}{\minidx}$.
%
From $\tau_{\minidx+1} \models \neg \dattreq{\tau_{\minidx}}{\minidx}$ and the
fact that, by Lemma~\ref{thm:tau}, $\mu$ lexicographically maximizes
$\dcala{}$, we derive that
$\vinonan \wedge \tau_{\minidx} \wedge \dattreq{\tau_{\minidx}}{\minidx}$ is unsatisfiable.
Because $\tau_{\minidx} \subset \tau_{\minidx+1}' \subseteq \mu'$ and
$\tau_{\minidx+1}' \models \dattreq{\tau_{\minidx}}{\minidx}$, we conclude
that $\vinonan \wedge \mu' \models \false$ and that $\calm'$ cannot be a
satisfiable model of $\vinonan$, contradicting the initial assumption.

%%%%%%%%%
%%%%%%%%%
%%%%%%%%%

In the second case, $\tau_{\minidx+1} \models \dattreq{\tau_{\minidx}}{\minidx}$
and $\tau_{\minidx+1}' \models \neg \dattreq{\tau_{\minidx}}{\minidx}$.
%
Given that $\dattreq{\tau_{\minidx}}{\minidx} \defas (\costbit{\minidx} = \dattrbit{\tau_{\minidx}}{\minidx})$,
we know that $\tau_{\minidx+1} \models (\costbit{\minidx} = \dattrbit{\tau_{\minidx}}{\minidx})$.
%
By Definition~\ref{def:dattr}, the dynamic attractor for \cost wrt. $\tau_{\minidx}$,
i.e. $\dattr{\tau_{\minidx}}$, is the smallest \fp value different from
$\nan$ s.t. the $\minidx$ most-significant bits of $\dattr{\tau_{\minidx}}$ have
the same value as the $\minidx$ most-significant bits of $\cost$ in $\tau_{\minidx}$.
%
Therefore, for every pair of complete truth assignments $\gamma$
and $\gamma'$ s.t. both $\gamma$ and $\gamma'$ satisfy $\vinonan$,
$\gamma$ extends $\tau_{\minidx+1}$ and $\gamma'$ extends $\tau_{\minidx+1}'$,
we have that $\gamma(\cost) \leq \gamma'(\cost)$.
%
Since $\tau_{\minidx+1} = \restr{\mu}{\minidx+1}$ and $\tau_{\minidx+1}' = \restr{\mu'}{\minidx+1}$,
it follows that $\calm'(\cost) \not< \calm(\cost)$, contradicting the initial assumption.

(Dual for maximization)
\hfill $\Box$
\end{proof}

